PerfCoder: Large Language Models for Interpretable Code Performance Optimization

Large language models (LLMs) have achieved remarkable progress in automatic code generation, yet their ability to produce high-performance code remains limited--a critical requirement in real-world software systems. We argue that current LLMs struggle not only due to data scarcity but, more importantly, because they lack supervision that guides interpretable and effective performance improvements. In this work, we introduce PerfCoder, a family of LLMs specifically designed to generate performance-enhanced code from source code via interpretable, customized optimizations. PerfCoder is fine-tuned on a curated collection of real-world optimization trajectories with human-readable annotations, and preference-aligned by reinforcement fine-tuning using runtime measurements, enabling it to propose input-specific improvement strategies and apply them directly without relying on iterative refinement. On the PIE code performance benchmark, PerfCoder surpasses all existing models in both runtime speedup and effective optimization rate, demonstrating that performance optimization cannot be achieved by scale alone but requires optimization stratetgy awareness. In addition, PerfCoder can generate interpretable feedback about the source code, which, when provided as input to a larger LLM in a planner-and-optimizer cooperative workflow, can further improve outcomes. Specifically, we elevate the performance of 32B models and GPT-5 to new levels on code optimization, substantially surpassing their original performance.

==> figure/extraction.tex <==
\begin{figure*}[h]
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{The optimization strategy extraction prompt template.}
  \label{fig-extraction}
    \vspace{-5mm}
\end{figure*}


==> section/6-ack.tex <==
\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2025/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

==> section/method_backup.tex <==
\section{Method}
\label{sec:method}

This section details the design of \textbf{PerfCoder}, a strategy-aware language model architecture for source code performance optimization. An illustration of the whole process is shown in Figure~\ref{fig-illu}. In contrast to prior work that focuses primarily on behavioral imitation or reinforcement through runtime metrics, PerfCoder centers its optimization learning around structured strategy induction. Our pipeline begins by reconstructing the PIE dataset into a strategy-aligned corpus $\mathcal{D}_{\text{ref}}$, enabling principled optimization supervision. From this, we extract and categorize transformation strategies into a structured space $\mathcal{S}$, construct a balance-aware training subset $\mathcal{D}_b$, and fine-tune a model using a structured single-step format that captures both strategy and implementation within a unified output.


\input{figure/illu}

\subsection{Dataset Reconstruction and Quality Enhancement}

Let $\mathcal{D}_{\text{PIE}} = \{(x^{(u,p)}_{\text{slow}}, x^{(u,p)}_{\text{fast}})\}$ represent the original PIE dataset, where each tuple comprises two code submissions by user $u$ to problem $p \in \mathcal{P}$: $x^{(u,p)}_{\text{slow}}$, an earlier version, and $x^{(u,p)}_{\text{fast}}$, a later version that improves execution time by at least 10\%.

Despite offering a rich source of real-world optimization behavior, the original dataset introduces inconsistencies incompatible with strategy-centric learning. Specifically, the dataset may contain overlapping optimization paths—e.g., $(v_1, v_2)$ and $(v_1, v_3)$—without a clearly defined optimization endpoint. This multiplicity diffuses the learning signal, exposing the model to both partial and final optimizations without guidance on which transformation is definitive.

Additionally, while users typically improve their own submissions, the absolute quality of final versions may vary widely across users. A user achieving strong relative gains may still submit code that performs significantly worse than peer solutions, introducing noise in optimization targets and diluting the model’s understanding of effective optimization.

To impose strategic clarity and performance grounding, we construct a refined dataset $\mathcal{D}_{\text{ref}}$ through a two-stage filtering and correction process.

In the first stage, we restrict targets to final submissions:
\begin{equation}
    \mathcal{D}_{\text{ref}} = \left\{(x^{(u,p)}_{\text{slow}}, x^{(u,p)}_{\text{fast}}) \in \mathcal{D}_{\text{PIE}} \;\middle|\; x^{(u,p)}_{\text{fast}} = x^{(u,p)}_{\text{final}} \right\},
\end{equation}
where $x^{(u,p)}_{\text{final}}$ denotes the last submission from user $u$ for problem $p$.

In the second stage, we adjust targets when a user’s final code falls substantially below the best available performance for the problem. Let $T(\cdot)$ denote the runtime function and $x^{(p)}_{\text{best}}$ the globally fastest solution for problem $p$. If:
\begin{equation}
    T(x^{(u,p)}_{\text{final}}) > 2 \cdot T(x^{(p)}_{\text{best}}),
\end{equation}
we replace $x^{(u,p)}_{\text{fast}}$ with $x^{(p)}_{\text{best}}$ in the pair. This ensures the model learns to target performance-competitive implementations, not merely user-local improvements. A dataset overview is given in Table~\ref{tab-data}.


\input{table/data}

\subsection{Optimization Strategy Extraction and Categorization}

The refined dataset $\mathcal{D}_{\text{ref}}$ provides well-defined, high-quality optimization trajectories. For each pair $(x^{(u,p)}_{\text{slow}}, x^{(u,p)}_{\text{fast}}) \in \mathcal{D}_{\text{ref}}$, we extract a set of optimization strategies $\mathbf{s}^{(u,p)} = \{s_1, \dots, s_k\}$ that describe the transformations applied. The union over all user-problem pairs yields the full strategy corpus:
\[
    \mathcal{S} = \bigcup_{(u,p)} \mathbf{s}^{(u,p)}.
\]

Each strategy \( s_i \in \mathbf{s}^{(u,p)} \) is modeled as a structured tuple:
\begin{equation}\label{equ-stra}
    s_i = (\texttt{name}_i, \texttt{desc}_i),
\end{equation}
where \( \texttt{name}_i \in \mathcal{V}_{\text{name}} \) is a short, canonical identifier of the optimization technique (e.g., \texttt{Data Structure Selection}), and \( \texttt{desc}_i \in \mathcal{V}_{\text{desc}} \) is a natural language explanation detailing the rationale and performance implications of applying this strategy to \( x^{(u,p)}_{\text{slow}} \). For example:
\[
    s = (\text{Data Structure Selection}, \text{“The original code uses a } \texttt{std::string} \text{..."})
\]
This representation disentangles what transformation is applied from why it is effective, promoting interpretability and strategy generalization across code contexts.

To extract these strategies, we use an instruction-tuned language model $f_\theta$ (Qwen2.5-32B-Inst) in a three-phase process:

\paragraph{(1) Direct Extraction.}
We prompt $f_\theta$ to generate the strategy set for each optimization pair:
\begin{equation}
    \mathbf{s}^{(u,p)} = f_\theta(x^{(u,p)}_{\text{slow}}, x^{(u,p)}_{\text{fast}}).
\end{equation}
The model outputs each strategy in the structured format above, ensuring that both high-level abstraction (\texttt{name}) and contextual reasoning (\texttt{desc}) are captured.

\paragraph{(2) Deduplication and Categorization.}
Due to lexical variation, strategies across $\mathcal{S}$ may redundantly express equivalent techniques. We normalize by technique name to produce a unique set $\mathcal{S}_{\text{uniq}}$ (with 60,650 entries). To structure the space, we define a taxonomy of categories $\mathcal{C} = \{c_1, \dots, c_{15}\}$ by concluding categories from 1,000 random strategy names and classifying the remainder:
\begin{equation}
    \text{Classify}(\texttt{name}_i) \rightarrow c_j \in \mathcal{C}.
\end{equation}
This enables downstream filtering, balancing, and interpretability. Notably, over 90.27\% of extracted strategies align with this taxonomy.

\paragraph{(3) Category-Guided Re-Extraction.}
To construct our fine-tuning dataset, we reprocess each pair $(x^{(u,p)}_{\text{slow}}, x^{(u,p)}_{\text{fast}})$ using prompts conditioned on the predefined category set $\mathcal{C}$. The extractor is instructed to identify each optimization strategy applied in the transformation and assign it to a category in $\mathcal{C}$, producing a structured tuple $(\texttt{name}, \texttt{desc})$ for each. The description \texttt{desc} is required to include a context-specific explanation that justifies the strategy's applicability based on the properties of $x^{(u,p)}_{\text{slow}}$. This yields:
\begin{equation}
    \mathcal{D}_{\text{cat}} = \left\{(x^{(u,p)}_{\text{slow}}, \mathbf{s}^{(u,p)}, x^{(u,p)}_{\text{fast}})\right\},
\end{equation}
where $s^{(u,p)}$ include category names and corresponding pair-specific strategy explanation as shown in Equation~\ref{equ-stra}. Figure~\ref{fig-example} presents an example set of optimization strategies extracted for a specific instance of slow-performing code.

The incorporation of contextual, slow-code-grounded explanations in each \( \texttt{desc}_i \) reinforces the causal connection between the proposed strategy and its expected performance impact. This structure is critical for training strategy-aware optimization models that are not only accurate, but interpretable and modular in their reasoning.


\subsection{Balanced Strategy Sampling}

Although $\mathcal{C}$ provides structural regularization, category frequency remains skewed. To prevent bias toward common strategies, we define a rarity-weighted score for each annotated pair:
\begin{equation}
    S^{(u,p)} = \frac{1}{k} \sum_{i=1}^{k} \frac{1}{f(s_i)},
\end{equation}
where $f(s_i)$ is the frequency of strategy $s_i$ in $\mathcal{D}_{\text{cat}}$.

We rank all pairs per problem by $S^{(u,p)}$ and select the top-ranked entries in a round-robin fashion to construct a balanced training set:
\begin{equation}
    \mathcal{D}_b \subset \mathcal{D}_{\text{cat}}, \quad |\mathcal{D}_b| = 5000.
\end{equation}
This promotes long-tail strategy coverage and ensures broader generalization during fine-tuning. \blue{The distributions of the refined and the balanced data can be found in supplementary material.}



\subsection{Single-Step Optimization Format}

To support flexible training and inference, we adopt a structured, single-step generation format. During fine-tuning, we optimize the standard causal language modeling loss over both the extracted strategy sequence and the optimized code. Given an instruction and slow code $x^{(u,p)}_{\text{slow}}$, the model $g_\phi$ is trained to auto-regressively generate the full target sequence:
\begin{equation}
    y^{(u,p)} = \texttt{[SUGG/]} \mathbf{s}^{(u,p)} \texttt{[/SUGG]} \texttt{[OPT/]} x^{(u,p)}_{\text{fast}} \texttt{[/OPT]}.
\end{equation}

\blue{The training loss is defined as:
\begin{equation}
    \mathcal{L}_{\text{LM}} = - \sum_{t=1}^{|y^{(u,p)}|} \log P(y_t \mid y_{<t}, \text{instruction}, x^{(u,p)}_{\text{slow}}; \phi),
\end{equation}
where $P(y_t \mid \cdot)$ is the model’s predicted token distribution at position $t$, and $\phi$ denotes model parameters.
}

This single-step design ensures that the model learns to jointly predict high-level optimization strategies and corresponding code refinements in a coherent sequence. It also enables two distinct inference modes: in strategy-only mode, generation is truncated at \texttt{[/SUGG]}, producing an interpretable plan without emitting code.

Crucially, this format supports integration with stronger, general-purpose LLMs (e.g., GPT-4, CodeLlama-70B) by allowing PerfCoder to act as a lightweight planning module. The generated strategy $\mathbf{s}^{(u,p)}$ can guide these external models to produce optimized implementations, effectively injecting optimization awareness into LLMs that were not explicitly trained for performance-critical tasks. This decoupled architecture enhances PerfCoder's generalizability and practical impact across real-world code optimization workflows.


\input{figure/example}
